Rayleigh Quotient Graph Neural Networks for Graph-level Anomaly Detection

Graph-level anomaly detection has gained significant attention as it finds applications in various domains, such as cancer diagnosis and enzyme prediction. However, existing methods fail to capture the spectral properties of graph anomalies, resulting in unexplainable framework design and unsatisfying performance. In this paper, we re-investigate the spectral differences between anomalous and normal graphs. Our main observation shows a significant disparity in the accumulated spectral energy between these two classes. Moreover, we prove that the accumulated spectral energy of the graph signal can be represented by its Rayleigh Quotient, indicating that the Rayleigh Quotient is a driving factor behind the anomalous properties of graphs. Motivated by this, we propose Rayleigh Quotient Graph Neural Network (RQGNN), the first spectral GNN that explores the inherent spectral features of anomalous graphs for graph-level anomaly detection. Specifically, we introduce a novel framework with two components: the Rayleigh Quotient learning component (RQL) and Chebyshev Wavelet GNN with RQ-pooling (CWGNN-RQ). RQL explicitly captures the Rayleigh Quotient of graphs and CWGNN-RQ implicitly explores the spectral space of graphs. Extensive experiments on 10 real-world datasets show that RQGNN outperforms the best rival by 6.74% in Macro-F1 score and 1.44% in AUC, demonstrating the effectiveness of our framework. Our code is available at https://github.com/xydong127/RQGNN.

==> table/tab-CB-loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\begin{tabular}{cc|cc}
\hline \hline 
Datasets                 & Metrics & ours   & no CB  \\ \hline 
\multirow{2}{*}{MCF-7}   & AUC     & 0.8354 & 0.8239 \\  
                         & F1      & 0.7394 & 0.7293 \\ \hline
\multirow{2}{*}{MOLT-4}  & AUC     & 0.8316 & 0.8228 \\  
                         & F1      & 0.7240 & 0.7361 \\ \hline
\multirow{2}{*}{PC-3}    & AUC     & 0.8782 & 0.8713 \\ 
                         & F1      & 0.7184 & 0.7544 \\ \hline
\multirow{2}{*}{SW-620}  & AUC     & 0.8550 & 0.8504 \\  
                         & F1      & 0.7335 & 0.7081 \\ \hline
\multirow{2}{*}{NCI-H23} & AUC     & 0.8680 & 0.8539 \\ 
                         & F1      & 0.7214 & 0.7340 \\ \hline
\multirow{2}{*}{OVCAR-8} & AUC     & 0.8799 & 0.8563 \\ 
                         & F1      & 0.7215 & 0.7126 \\ \hline
\multirow{2}{*}{P388}    & AUC     & 0.9023 & 0.8883 \\ 
                         & F1      & 0.7963 & 0.7897 \\ \hline
\multirow{2}{*}{SF-295}  & AUC     & 0.8825 & 0.8792 \\ 
                         & F1      & 0.7416 & 0.7074 \\ \hline
\multirow{2}{*}{SN12C}   & AUC     & 0.8861 & 0.8803 \\ 
                         & F1      & 0.7660 & 0.7554 \\ \hline
\multirow{2}{*}{UACC257} & AUC     & 0.8724 & 0.8537 \\
                         & F1      & 0.7362 & 0.7095 \\ \hline 
                         \hline 
\end{tabular}
\caption{Ablation study for class balanced loss}
\label{tab:class balanced loss}
\end{table}

==> table/tab-graph-classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\small\centering
\begin{tabular}{cc|cc|cc|cc}
\hline \hline
Datasets                 & Metrics & TVGNN & TVGNN-CB & Gmixup & Gmixup-CB & GMT & GMT-CB \\ \hline
\multirow{2}{*}{MCF-7}   & AUC     & 0.7180        & 0.7309   & 0.6954         & 0.6984    & 0.7706      & 0.7479 \\  
                         & F1      & 0.5594        & 0.5608   & 0.4779         & 0.4779    & 0.4784      & 0.4784 \\ \hline
\multirow{2}{*}{MOLT-4}  & AUC     & 0.7159        & 0.7574   & 0.6232         & 0.6644    & 0.7606      & 0.6226 \\  
                         & F1      & 0.4916        & 0.5793   & 0.4789         & 0.4789    & 0.4814      & 0.4794 \\ \hline
\multirow{2}{*}{PC-3}    & AUC     & 0.7974        & 0.7025   & 0.6908         & 0.6592    & 0.7896      & 0.7877 \\ 
                         & F1      & 0.6206        & 0.5331   & 0.4852         & 0.4852    & 0.4853      & 0.4853 \\ \hline
\multirow{2}{*}{SW-620}  & AUC     & 0.7326        & 0.7332   & 0.6479         & 0.6202    & 0.7467      & 0.7620 \\ 
                         & F1      & 0.5365        & 0.5547   & 0.4844         & 0.4844    & 0.4874      & 0.4847 \\ \hline
\multirow{2}{*}{NCI-H23} & AUC     & 0.7782        & 0.7810   & 0.7324         & 0.6793    & 0.8030      & 0.7808 \\ 
                         & F1      & 0.5520        & 0.5484   & 0.4869         & 0.4869    & 0.4869      & 0.4869 \\ \hline
\multirow{2}{*}{OVCAR-8} & AUC     & 0.7653        & 0.6891   & 0.5663         & 0.6591    & 0.7692      & 0.7713 \\ 
                         & F1      & 0.5406        & 0.5155   & 0.4869         & 0.4869    & 0.4868      & 0.4868 \\ \hline
\multirow{2}{*}{P388}    & AUC     & 0.7957        & 0.7757   & 0.6516         & 0.6562    & 0.8495      & 0.8638 \\ 
                         & F1      & 0.5557        & 0.5549   & 0.4856         & 0.4856    & 0.6583      & 0.6268 \\ \hline
\multirow{2}{*}{SF-295}  & AUC     & 0.7346        & 0.7722   & 0.6471         & 0.7070    & 0.7992      & 0.8004 \\ 
                         & F1      & 0.4935        & 0.5779   & 0.4866         & 0.4866    & 0.4871      & 0.4871 \\ \hline
\multirow{2}{*}{SN12C}   & AUC     & 0.7441        & 0.7710   & 0.7211         & 0.7017    & 0.7919      & 0.7985 \\ 
                         & F1      & 0.5437        & 0.5736   & 0.4871         & 0.4871    & 0.4874      & 0.4875 \\ \hline
\multirow{2}{*}{UACC257} & AUC     & 0.7410        & 0.7450   & 0.6564         & 0.6097    & 0.7735      & 0.7845 \\ 
                         & F1      & 0.5373        & 0.5330   & 0.4904         & 0.4904    & 0.4894      & 0.4895 \\ \hline \hline
\end{tabular}
\caption{Substitute Cross Entropy loss with Class Balanced loss for graph classification models}
\label{tab:graph classification}
\end{table}
